VEU-Bench: Towards Comprehensive Understanding of Video Editing

Widely shared videos on the internet are often edited. Recently, although Video Large Language Models (Vid-LLMs) have made great progress in general video understanding tasks, their capabilities in video editing understanding (VEU) tasks remain unexplored. To address this gap, in this paper, we introduce VEU-Bench (Video Editing Understanding Benchmark), a comprehensive benchmark that categorizes video editing components across various dimensions, from intra-frame features like shot size to inter-shot attributes such as cut types and transitions. Unlike previous video editing understanding benchmarks that focus mainly on editing element classification, VEU-Bench encompasses 19 fine-grained tasks across three stages: recognition, reasoning, and judging. To enhance the annotation of VEU automatically, we built an annotation pipeline integrated with an ontology-based knowledge base. Through extensive experiments with 11 state-of-the-art Vid-LLMs, our findings reveal that current Vid-LLMs face significant challenges in VEU tasks, with some performing worse than random choice. To alleviate this issue, we develop Oscars, a VEU expert model fine-tuned on the curated VEU-Bench dataset. It outperforms existing open-source Vid-LLMs on VEU-Bench by over 28.3% in accuracy and achieves performance comparable to commercial models like GPT-4o. We also demonstrate that incorporating VEU data significantly enhances the performance of Vid-LLMs on general video understanding benchmarks, with an average improvement of 8.3% across nine reasoning tasks.

==> sec/0_abstract.tex <==
\begin{abstract}
Video content is increasingly dominant, rich in high-density, multi-modal information. While Video Language Models (ViLMs) have advanced general video understanding tasks like question answering and captioning, their ability to handle video editing tasks remains untested. Video editing demands complex spatial-temporal comprehension and serves as both a critical application and a comprehensive evaluation of ViLMs. To address this gap, we introduce OSCAR, a comprehensive benchmark for evaluating ViLMs on video editing tasks. OSCAR features multi-level tasks across recognition, reasoning, and recommendation stages, covering shot elements, camera motion, editing techniques, and transition effects. We collected and annotated a high-quality dataset and thoroughly evaluated mainstream ViLMs on these tasks. Our findings reveal that current ViLMs struggle with professional video editing methods. By fine-tuning ViLMs on our curated video editing dataset, we developed an expert model that outperforms existing state-of-the-art models on the OSCAR benchmark by over XXX\% accuracy. We also demonstrate that incorporating video editing data enhances performance on general video evaluation benchmarks. Our contributions are threefold: (1) We introduce OSCAR, a benchmark for evaluating ViLMs on video editing tasks and provide high-quality data for future research. (2) We assess current state-of-the-art ViLMs, uncovering their limitations in handling professional video editing tasks. (3) We show that fine-tuning ViLMs on our dataset significantly improves performance on both OSCAR and general video benchmarks.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% introduce video editing task, state the lack of attention and research on such domain.
Video has gradually become a dominant data form, containing high-density information integrated from various modalities. Consequently, recent advances in the computer vision community have shown increased attention to the video domain, especially in general video understanding\cite{} and generation\cite{}. However, although the majority of online videos are edited, efforts to understand the video editing process remain insufficient. Understanding the basic editing components and applying these concepts for better video production remain unexplored. Moreover, most prior work\cite{} related to editing tasks focuses on the movie industry, while nowadays short videos on social media are becoming increasingly prevalent. 

% NEED CLEAR DEFINITION of "video editing" discussed in this work VERY IMPORTANT

% Is it necessary to add this line?
% To clarify, in this context, video editing refers to traditional video editing tasks originating from the film industry, not the content-altering type of video editing tasks\cite{}.

% introduce video-llm and it's advance, relation to the video editing
Thanks to breakthroughs in large language models (LLMs)\cite{}, a series of video language models (ViLMs)\cite{} have been proposed to expand the boundaries of video understanding tasks, achieving remarkable performance on a range of general video understanding tasks, including video question answering (VideoQA)\cite{}, video captioning\cite{}, and video reasoning\cite{}. With the development of ViLMs, several video benchmarks\cite{} have been proposed to evaluate models’ video understanding abilities from different perspectives. These benchmarks mainly focus on establishing general video understanding evaluation protocols. However, they often overlook the specific challenges posed by video editing tasks.

While ViLMs’ abilities have been measured through existing benchmarks, their capacity to handle video editing tasks has not been evaluated. Video editing is a time-based medium, requiring both spatial and temporal, static and dynamic understanding of multi-video data, which perfectly matches the properties of video models. Moreover, “video editing is also a language with structured information”\cite{}, making it suitable for LLMs to understand and interpret. Therefore, video editing tasks are naturally suited for ViLMs. Not only can ViLMs offer better solutions to automatic video editing tasks, but video editing tasks can also comprehensively evaluate the abilities of ViLMs.

% existing video editing tasks, it's shortcoming
Dating back to the era of end-to-end methods, several tasks have been proposed to explore the potential to handle different aspects of editing tasks. However, the need for a comprehensive editing benchmark covering various dimensions and levels of tasks remains unmet. Additionally, due to the limited label space of end-to-end methods, most proposed tasks are confined to classification within constrained labels, lacking open-vocabulary reasoning and open-ended understanding. These capabilities are vital for video editing tasks that require creativity and open-minded reasoning.

% our proposed benchmark
To overcome the aforementioned obstacles, we propose OSCAR, a comprehensive video editing benchmark that thoroughly categorizes the elements and dimensions of video editing tasks. It introduces multi-level tasks that encompass three stages: recognition, reasoning, and recommendation. The benchmark covers various aspects such as shot elements, camera motion, editing techniques, and transition effects. We have collected, organized, and annotated a comprehensive and high-quality dataset, and thoroughly evaluated the performance of all mainstream ViLMs on video editing tasks, including training data discussions to fully understand the underlying challenges. Beyond evaluating models’ performance on domain-related tasks, we propose a decomposed correlation to project models’ performance on video editing tasks to general video abilities, enabling evaluation of ViLMs from both general and domain-specific perspectives.

Besides the high-quality evaluation samples, we also collect large-scale video-editing-related data to develop an expert ViLM well-equipped with video editing knowledge, showing outstanding performance across various tasks on the OSCAR benchmark. Moreover, OSCAR’s performance reveals the value of editing-related video data by showing improvements on general video evaluation benchmarks. Detailed ablation studies further demonstrate the effectiveness of the correlation projection, making this kind of data necessary as part of video pre-training and fine-tuning sources.

Our contributions can be summarized as follows:
\begin{itemize}
\item We introduce OSCAR, a comprehensive benchmark designed to evaluate ViLM's performance on video editing tasks and high-quality video editing data for further research works.
\item We assessed current state-of-the-art ViLM, fully investigated the intrinsic editing knowledge and found that they struggle with more professional video editing methods, showing limitations on xxx even with limited video length.
\item By fine-tuning on our curated dataset, we demonstrate that ViLM can indeed grasp the understanding of editing component, surpassing existing state-of-the-art models by over xxx accuracy on OSCAR and general video benchmark.
\end{itemize}


% editing task is better with video-llm, both for task and model
% editing task represent some high-level understanding ability, intergration of multi-dimension base ability
% editing task-video generation

% contribution
% 1. benchmark, tool & standard evaluate multi-level(recognize, reasoing ?recommandation/high-level judge, score)-multi-dimension(intra-frame inter-shot)
% 2. Fully analyze and explore the intrinsic editing knowledge lies in the video-llm, video-llm 
% 3. Finetune a editing-speific expert, task good, improve ability on other general benchmarks.

% 1. former existing tasks, but limitation, e2e model classification, no open-vocabulary
% 2. benchmark only limited to specific persepctive, limit comprehensive and fully-covered dimensions
% 3. decompose video editing task into multi-level and multi-dimension tasks, offer a more reasonable benchmark to evaluate and redefine the task
% 4. evaluate video-llms's problem and potential on such task, relationship with general/base ability
% 5. finetune a model, task-specific performance improvement and general benchmark improvement, temporal/dynamic information/ability(on-hold, depends on experiment output)

==> sec/2_relatedwork.tex <==
\section{Related Work}
\noindent
\textbf{Video Editing Task.} Video editing encompasses a range of complexities, extending beyond intra-frame manipulations addressed by pixel-level editing techniques\cite{}. Editing video clips\cite{wohl2002editing} represents a particularly demanding task within video understanding, requiring a nuanced comprehension of both content and editing principles. However, progress in this area has been hampered by several factors: the scarcity of large, publicly available, high-quality datasets; the subjective nature of evaluating editing quality; and limitations in the capabilities of existing video understanding models. Prior research has explored various facets of video editing. Some studies have focused on analyzing and understanding technical aspects like camera shot settings\cite{argaw2022anatomy, vacchetti2022movie, huang2020movienet}, transitions between shots\cite{shen2022autotransition}, visual effects\cite{gu2024edit3k,xu2024beyond}, and cut types\cite{pardo2022moviecuts, chen2023match}. Most of these works adopted end-to-end learning frameworks that limited to single perspective. Moreover, these approaches often lack the ability to effectively address the subjective nature of video editing, primarily focusing on recognition rather than high-level understanding tasks.

\noindent
\textbf{Video-LLM}
Recently, with the success of Large Language Models (LLMs) and Large Vision-Language Models (LVLMs), the video domain has witnessed a significant leap forward, marked by the introduction of a series of pioneering Video Language Models (ViLMs) \cite{cheng2024videollama,fei2024video,zhang2024internlm,chen2024far,yao2024minicpm,wang2024qwen2,xue2024longvila}. Building on the architecture of the most representative model, LLaVA, and incorporating either multi-image training strategies or video-specific module designs, these models have substantially raised the bar for video understanding systems. Concurrently, several proprietary commercial models \cite{team2023gemini, wu2024gpt} have demonstrated superior video understanding capabilities. While these models excel in general video understanding tasks, their potential applications in video editing tasks remain largely underestimated. \cite{xu2024beyond} explored VideoLLM’s capability in recognizing and analyzing edited videos, but a comprehensive evaluation of ViLMs in video editing tasks—especially those that involve deeper intrinsic knowledge and novel editing scenarios—remains absent. The unique strengths of VideoLLMs, the rich internal knowledge and powerful learning capacity, suggest they could be particularly well-suited for more complex video editing tasks that go beyond simple close-set recognition. However, this area remains largely unexplored.

\noindent
\textbf{Video Benchmark}
% existing benchmark
% problem? Relation to the editing?
As Video Language Models (ViLM) continue to evolve, several video-related benchmarks \cite{} have been proposed to evaluate and comprehensively assess the capabilities of ViLM. Many of these benchmarks focus on general understanding and reasoning abilities, classifying various dimensions to decompose the evaluation process and cover multiple perspectives, including perception and reasoning across both spatial and temporal dimensions. While these benchmarks provide valuable insight into the general capabilities of ViLM, they fall short in assessing the model’s intrinsic knowledge related to video editing and its potential in task require support both technical and creativity. Also, despite increasing attention on long-term video analysis benchmarks, the nuanced understanding of interactions between short video clips remains largely underexplored. Video editing and judging tasks provide an ideal avenue for evaluating this dimension. Evaluating the ability of ViLM to understand and assist in video editing can deepen the insight for its application potential and comprehensive ability under complex scenario.


==> sec/3_benchmark.tex <==
\section{Benchmark}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{Figure/data_pipeline.pdf}
    \caption{dataset construction pipeline}
    \label{fig:dataset_pipeline}
\end{figure*}
% give the definition of different dimensions through intra-frame, intra-shot inter-frame and intra-shot
% give definition of different level of editing task from component recognition to reasoning and ultimately judging, recommendation and score. 
% last level is hard to set, we can propose some possible solution. left the plan as next-step research.
\subsection{Multi dimensions and level of benchmark}
Video editing is conducted based on raw footage. The basic unit that compose final edited video can be divided into noun and verb, where noun refer to static intra-frame attribute and verb refer to dynamic editing techniques. Former include various shot attributes like shot size shot location and shot angle. Latter contain intra-shot component like shot motion and shot speed and inter-shot perspective like cut type and transition. Therefore, We divide video editing task into 10 dimensions. At the same time, to evaluate the model’s capabilities at different levels in video editing tasks, this benchmark divides the tasks into three dimensions: recognize, reason, and judge. It progressively tests the model’s performance on video editing tasks ranging from simple to complex. 

\noindent
\textbf{Dimensions of editing task} 
The proposed benchmark contain 10 dimensions, covering intra-frame, inter-frame \& intra-shot and inter-shot component of editing tasks.

\textbf{Intra-frame} (1) shot size: Defined as how much of the setting or subject is displayed within a given shot. Include five categories: extreme wide, wide, medium, close-up, extreme close-up. (2) shot angle the location where the camera is placed to take a shot. Include five categories: aerial, overhead, eye level, high angle, low angle. (3)shot location: the environment where the shot is taken. Inlucde two categories: indoor, outdoor. (4) shot subject: the main subject featured or conveyed in the shot. (5) shot type: The composition of a shot in terms of the number of featured subjects and their physical relationship to each other and the camera. Include: (shot type category need to be discussed). (6) shot color: the alterations made to the color of a video clip used to create a specific visual tone or mood. include warm, middle, cold.\textbf{Inter-frame \& Intra-shot} (1) shot motion: The movement of the camera when taking a shot. Include pan, tilt, locked, zoom, handheld. (2) Shot speed: Change of shot speed compared to normal video clips. Include slow, fast and normal.\textbf{Inter-shot} (1) cut: Composed of two adjacent shots and the transition between them, without special visual effects and achieved by pure cutting. Include: cut-on-action, cross cut, emphasis cut, cut away, reaction cut, smash cut, match-cut. (2) Transition: Move from one shot to the next with special visual effects, creating a smooth or intentional visual effect as one clip changes to another. Include: (transition category need to be modified).

\noindent
\textbf{Levels of editing task}
VEditBench define three levels of editing tasks, measuring model's capacity on editing tasks from recognizing basic editing component to high level reasoning and judging.  \textbf{Recognition}: in the level 1 recognition tasks, model should be able to tell the difference between different category of each dimensions. This level not only exam the basic understanding of editing task but also offer comparison of Vid-LLM with traditional end2end model. \textbf{Reasoning}: this level of task require model to give detailed reasoning of each dimension, including video-specific key attribution reasoning and multi dimension component joint reasoning. It is notable that as the level raise, there will be interaction among dimensions that result in more complex tasks. \textbf{Judging}: the ultimate goal of AI assisted task is to enable automatic editing, hence in this level the benchmark require model to tell the function, benefit and drawbacks of inter-shot dimensions based on video content and basic shot attributions. Once model can give high quality judge on video input, then it is supposed to give recommendation and even finish editing process on its own, reaching the final destination. 

\subsection{Dataset construction}
\noindent
\textbf{Video Source} Since we focus on building a benchmark for understanding video editing, we have constructed VEditBench by collecting and restructuring data from previous video editing-related datasets\cite{}. Specifically, AVE mainly provides intra-frame and inter-frame intra-shot dimension video data, which is used to understand the fundamental video editing elements within each shot. Moviecut and AutoTransition primarily offer inter-shot video data. Some prior works (citation) have also aimed to understand video editing elements, but since they are not publicly available, they are not considered here. These three datasets together contain approximately NK videos, with lengths predominantly around xx, covering most of the basic elements in editing. Additionally, since the sources of these datasets primarily include movies and social media, the content of the videos ensures substantial semantic diversity. Details on the distribution of original dataset video data are provided in the appendix.

\noindent
\textbf{dimension expand} Beside existing tasks, to expand the dimensions, we xxx.

\noindent
\textbf{Automatic high-level annotation}


\subsection{Dataset Statistics}


\subsection{Evaluation Prompt Design}


==> sec/3_method.tex <==
\section{Method}


\subsection{How to Choose the proper visual Prompt}

==> tables/category_table.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{minipage}{\linewidth}
        \centering
        \begin{tabular}{cccc}
        \vspace{15pt}
        
            % First Row of Tables
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \begin{tabular}{l|cccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Shot Size Recognition}} \\
                    \cmidrule{2-6}
                    ~              & \textbf{EW} & \textbf{W} & \textbf{ECU} & \textbf{M} & \textbf{CU} \\
                    \midrule
                    Qwen2-VL       & 1                  & 82         & 32                      & 37            & 89             \\
                    Gemini-Pro     & 26                  & 28         & 87                      & 82            & 58             \\
                    \rowcolor{Gray!30} Oscars         & 92                  & 22         & 94                      & 72            & 61     \\
                    \bottomrule
                \end{tabular}
            \end{minipage} &
            \hspace{5pt}
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \begin{tabular}{l|ccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Shot Angle Recognition}} \\
                    \cmidrule{2-6}
                    ~ & \textbf{O} & \textbf{H} & \textbf{L} & \textbf{E} & \textbf{A} \\
                    \midrule
                    Qwen2-VL   & 63 & 0 & 29 & 82 & 79 \\
                    Gemini-Pro & 43 & 61 & 59 & 67 & 0 \\
                    \rowcolor{Gray!30}Oscars     & 76 & 20 & 35 & 63 & 68 \\
                    \bottomrule
                \end{tabular}
            \end{minipage} \\ 
            % Add vertical space between rows
        \end{tabular}
        \vspace{15pt}
        \begin{tabular}{cccc}
            % Second Row of Tables
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \begin{tabular}{l|ccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Shot Type Recognition}} \\
                    \cmidrule{2-6}
                    ~ & \textbf{Th} & \textbf{Tw} & \textbf{S} & \textbf{OTS} & \textbf{G} \\
                    \midrule
                    Qwen2-VL   & 75 & 79 & 76 & 0 & 72 \\
                    Gemini-Pro & 79 & 77 & 92 & 36 & 91 \\
                    \rowcolor{Gray!30}Oscars     & 85 & 76 & 86 & 47 & 71 \\
                    \bottomrule
                \end{tabular}
            \end{minipage} &
            \hspace{5pt}
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \begin{tabular}{l|ccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Shot Motion Recognition}} \\
                    \cmidrule{2-6}
                    ~ & \textbf{H} & \textbf{Z} & \textbf{L} & \textbf{T} & \textbf{P} \\
                    \midrule
                    Qwen2-VL   & 1 & 1 & 74 & 4 & 61 \\
                    Gemini-Pro & 25 & 32 & 74 & 19 & 29 \\
                    \rowcolor{Gray!30}Oscars     & 13 & 13 & 67 & 28 & 54 \\
                    \bottomrule
                \end{tabular}
            \end{minipage}
        \end{tabular}
        \vspace{15pt}
        \begin{tabular}{cccc}
            % Second Row of Tables
            \begin{minipage}[t]{\linewidth}
                \centering
                \begin{tabular}{l|ccccccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{8}{c}{\textbf{Shot Subject Recognition}} \\
                    \cmidrule{2-9}
                    ~ & \textbf{Object} & \textbf{Animal} & \textbf{Cartoon} & \textbf{Location} & \textbf{Limb} & \textbf{Human} & \textbf{Face} & \textbf{Text} \\
                    \midrule
                    Qwen2-VL   & 5  & 45 & 0    & 85 & 56 & 7  & 94 & 100 \\
                    Gemini-Pro & 66 & 59 & 0    & 77 & 58 & 85 & 98 & 100 \\
                    \rowcolor{Gray!30}Oscars     & 73 & 5  & 9 & 87 & 68 & 85 & 97 & 100 \\
                                        \bottomrule
                \end{tabular}
            \end{minipage} \\ 
        \end{tabular}
        \vspace{15pt}
        \begin{tabular}{cccc}
            % Second Row of Tables
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \begin{tabular}{l|cc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Shot Location Recognition}} \\
                    \cmidrule{2-3}
                    ~ & \textbf{Indoor Shot} & \textbf{Outdoor Shot}\\
                    \midrule
                    Qwen2-VL   & 75 & 79 \\
                    Gemini-Pro & 79 & 77 \\
                    \rowcolor{Gray!30}Oscars & 85 & 76 \\
                    \bottomrule
                \end{tabular}
            \end{minipage} &
            \hspace{5pt}
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \begin{tabular}{l|ccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Shot Motion Recognition}} \\
                    \cmidrule{2-6}
                    ~ & \textbf{H} & \textbf{Z} & \textbf{L} & \textbf{T} & \textbf{P} \\
                    \midrule
                    Qwen2-VL   & 1 & 1 & 74 & 4 & 61 \\
                    Gemini-Pro & 25 & 32 & 74 & 19 & 29 \\
                    \rowcolor{Gray!30}Oscars     & 13 & 13 & 67 & 28 & 54 \\
                    \bottomrule
                \end{tabular}
            \end{minipage} \\ 
        \end{tabular}
        \begin{tabular}{cccc}
            % Second Row of Tables
            \begin{minipage}[t]{\linewidth}
                \centering
                \begin{tabular}{l|cccccccc}
                    \toprule
                    \multirow{2}{*}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Cut Type Recognition}} \\
                    \cmidrule{2-8}
                    ~ & \textbf{match-cut} & \textbf{cross-cut} & \textbf{reaction cut} & \textbf{smash-cut} & \textbf{emphasis cut} & \textbf{cut-on-action} & \textbf{cut-away} \\
                    \midrule
                    Qwen2-VL   & 7 & 3 & 100 & 3 & 3 & 0 & 0 \\
                    Gemini-Pro & 7 & 3 & 3 & 67 & 33 & 57 & 53 \\
                    \rowcolor{Gray!30}Oscars     & 1 & 21 & 73 & 3 & 67 & 7 & 30 \\
                    \bottomrule
                \end{tabular}
            \end{minipage} \\ 
        \end{tabular}
    \end{minipage}
    \caption{Category-wise Performance comparison among Oscars, Qwen2-VL~\cite{wang2024qwen2} and Gemini~\cite{team2023gemini}.}
    \label{fig:multi_tables}
\end{figure*}
